The GN-z11-Flash Event Can be a Satellite Glint

Recently Jiang et al. reported the discovery of a possible short duration transient, detected in a single image, spatially associated with a z~11 galaxy. Jiang et al. and Kahn et al. suggested the transient originates from a Gamma-Ray Burst (GRB), while Padmanabhan & Loeb argued the flash is consistent with a supernova shock breakout event of a 300 M_sun population III star. Jiang et al. argued against the possibility that this event originated from light reflected off a satellite. Here we show that reflection of sunlight from a high-orbit satellite or a piece of space debris is a valid and reasonable explanation. As shown in recent works, the rate of point-like satellite reflections, brighter than 11th magnitude, is >10 deg^{-2} day^-1 near the equatorial plane. At higher declinations the rate is 5--50 times lower, but still significant: about four orders of magnitudes higher than the rate estimated for GRBs.

==> packages.tex <==
% \documentclass[a4paper,10pt]{article}
%\usepackage[left=2cm, right=3cm]{geometry}
% \usepackage{fullpage}

\makeatletter

%\usepackage{graphicx}

\usepackage{amsmath, amsthm, amssymb,amsfonts}
%\usepackage{mathrsfs}
%\usepackage{float}
%\restylefloat{figure}
\@ifclassloaded{emulateapj}{}{
\usepackage{euscript}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{pdfpages}
\usepackage{cite}
\numberwithin{equation}{section} % keeps equation numbering in section form
}

%\usepackage{natbib}
%\usepackage[backend=bibtex]{biblatex}
%\bibliographystyle{apj}
%\bibliography{P1640_AGES}

\usepackage{lipsum}

\usepackage{array}
\usepackage{multirow}
\usepackage{enumerate}

\usepackage{xspace}

\usepackage{color}
\usepackage{slashed}

\usepackage{xstring}
\usepackage{lineno}

\usepackage{url}

\usepackage{tikz}
\usetikzlibrary{shapes, arrows, shadows}

\usepackage[normalem]{ulem} % underline stuff (normalem leaves \emph command alone)

%\usepackage{makeidx}
\usepackage{tabularx}

\usepackage{listings}
\usepackage[T1]{fontenc} 
%\usepackage{upquote} 
\lstnewenvironment{matlab}{%
	\lstset{language=Matlab}%
}{}

% make sure PDF is loaded before PNG! 
\DeclareGraphicsExtensions{%
	.pdf,.PDF,%
	.png,.PNG,%
	.jpg,.mps,.jpeg,.jbig2,.jb2,.JPG,.JPEG,.JBIG2,.JB2}

%\newcommand{\pic}[2][1]{\begin{center}\includegraphics[width=#1\textwidth]{../pics/#2} \end{center}}


% taken from: http://tex.stackexchange.com/questions/99070/check-for-a-valid-file-before-using-includegraphics

\newif\ifgraphicexist

\catcode`\*=11
\newcommand\imagetest[1]{%
	\begingroup
	\global\graphicexisttrue
	\let\input@path\Ginput@path
	\filename@parse{#1}%
	\ifx\filename@ext\relax
	\@for\Gin@temp:=\Gin@extensions\do{%
		\ifx\Gin@ext\relax
		\Gin@getbase\Gin@temp
		\fi}%
	\else
	\Gin@getbase{\Gin@sepdefault\filename@ext}%
	\ifx\Gin@ext\relax
	\global\graphicexistfalse
	\def\Gin@base{\filename@area\filename@base}%
	\edef\Gin@ext{\Gin@sepdefault\filename@ext}%
	\fi
	\fi
	\ifx\Gin@ext\relax
	\global\graphicexistfalse
	\else 
	\@ifundefined{Gin@rule@\Gin@ext}%
	{\global\graphicexistfalse}%
	{}%
	\fi  
	\ifx\Gin@ext\relax 
	\gdef\imageextension{unknown}%
	\else
	\xdef\imageextension{\Gin@ext}%
	\fi 
	\endgroup 
	\ifgraphicexist
	\expandafter \@firstoftwo
	\else
	\expandafter \@secondoftwo
	\fi 
} 
\catcode`\*=12

%%%%%%%%%%%%%%

\newcommand{\putpic}[2]{\begin{minipage}[t]{#1\linewidth}\center\vspace{0pt}\includegraphics[width=1\linewidth]{#2}\end{minipage}}

\newcommand{\pic}[2][1]{ \imagetest{#2}{\putpic{#1}{#2}}{
							\imagetest{pics/#2}{\putpic{#1}{pics/#2}}{
								\imagetest{../pics/#2}{\putpic{#1}{../pics/#2}}{
									\imagetest{../../pics/#2}{\putpic{#1}{../../pics/#2}}{
										\textcolor{red}{!!cannot find \detokenize{#2}!!} } } } } 
					   }

\newcommand{\plot}[2][1]{\begin{center}\includegraphics[width=#1\textwidth]{\IfFileExists{plots/#2}{plots/#2}{../plots/#2}} \end{center}}

\newcommand{\cit}{$^\text{\textcolor{blue}{[citation needed]}}$\xspace}

\newcommand{\with}{\quad \text{with}\quad}

%\@ifundefined{code}{\newcommand{\code}[1]{\texttt{\detokenize{#1}}}}{}
\@ifundefined{code}{\newcommand{\code}[1]{\texttt{\lstinline[language=Matlab, basicstyle=\ttfamily, showstringspaces=false, breaklines=true, breakatwhitespace=true, prebreak=..., columns=flexible]!#1!}}}{}
\@ifundefined{terminal}{\newcommand{\terminal}{\code{$>>$\hspace{1ex}}}}{}
\@ifundefined{coded}{\newcommand{\coded}[1]{\vspace{0.1cm} \hspace{1em} \terminal \code{#1} \vspace{0.05cm}}}{}

\@ifundefined{class}{\newcommand{\class}[1]{\code{#1}}}{}

\@ifundefined{subtitle}{\newcommand{\subtitle}[1]{\vspace{0.3cm}\noindent\underline{#1}\vspace{0.1cm}}}{}

\@ifundefined{cvec}{\newcommand{\cvec}[1]{\code{vector$<$#1$>$}}}{}

\@ifundefined{comment}{\newcommand{\comment}[1]{\textcolor{gray}{#1}}}{}

\@ifundefined{note}{\newcommand{\note}[1]{\textcolor{red}{(\underline{NOTE:} #1)}}}{}{}

\@ifundefined{jump}{\newcommand{\jump}{\vspace{0.6cm}}}{}

\@ifundefined{apj}{\newcommand{\apj}{The Astrophysical Journal}}{}
\@ifundefined{aj}{\newcommand{\aj}{AstJ}}{}
\@ifundefined{apjl}{\newcommand{\apjl}{ApJ}}{}
\@ifundefined{aaps}{\newcommand{\aaps}{AAPS}}{}
\@ifundefined{nat}{\newcommand{\nat}{Nature}}{}
\@ifundefined{icarus}{\newcommand{\icarus}{Icarus}}{}
\@ifundefined{pasp}{\newcommand{\pasp}{PASP}}{}
\@ifundefined{physrep}{\newcommand{\physrep}{PhysRep}}{}
\@ifundefined{skytel}{\newcommand{\skytel}{S\& T}}{}
\@ifundefined{mnras}{\newcommand{\mnras}{MNRAS}}{}
\@ifundefined{bain}{\newcommand{\bain}{BAIN}}{}


\makeatother
